Characterizing High-Dimensional Optical Systems with Applications in Compressive Sensing and Quantum Data Locking

This University of Rochester Physics Ph.D. dissertation introduces concepts in compressive sensing, quantum entanglement, FMCW LiDAR, and quantum data locking. Additionally, the appendix serves as a thorough reference for those interested in applying the alternating direction method of multipliers (ADMM) to optimize an augmented Lagrangian and can easily be tailored to specific optimization problems. In particular, I show how fast Hadamard transforms and the ADMM can be used for $L^1$-minimization with different sparse-basis transforms along with total-variation minimization of both images and video. The simple examples given demonstrate how to minimize high-dimensional problems with little memory overhead. The original version of this dissertation can be accessed through ProQuest.

==> urpasmacros.tex <==
%
% urcsmacros
%
% author: Lawrence A. Crowl
% last updated: 28 April 1990
%
% BibTeX
%
\newcommand{\BibTeX}{{B\kern-.0833em{\sc ib}\kern-.1667em%
T\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX}}
%
% SLiTeX
%
\newcommand{\SliTeX}{{\rm S\kern-.06em{\sc l\kern-.035emi}\kern-.06em
T\kern -.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%
% UNIX
%
\newcommand{\UNIX}{{\sc Unix}}
%
% trademark
%
\newcommand{\trademark}{$^{\rm TM}$}
%
% singlespacing (for use in doublespaced documents)
%
\def\doublespacefactor#1#2{%
\newenvironment{singlespace}{\baselineskip #2\baselineskip}%
{\par \baselineskip #1\baselineskip}%
\par \baselineskip #1\baselineskip}
%
% various latin abbreviations
%
\def\adhoc{{\em ad hoc}}
\def\aposteriori{{\em a posteriori}}
\def\apriori{{\em a priori}}
\def\Cf{{\em Cf.}}
\def\cf{{\em cf.}}
\def\Eg{{\em E.g.}}
\def\eg{{\em e.g.}}
\def\etal{{\em et al.}}
\def\etc{{\em etc.}}
\def\Ibid{{\em Ibid.}}
\def\ibid{{\em ibid.}}
\def\Id{{\em Id.}}
\def\id{{\em id.}}
\def\Ie{{\em I.e.}}
\def\ie{{\em i.e.}}
\def\Loccit{{\em Loc.\ cit.}}
\def\loccit{{\em loc.\ cit.}}
\def\Opcit{{\em Op.\ cit.}}
\def\opcit{{\em op.\ cit.}}
\def\qv{{\em q.v.}}
\def\Qv{{\em Q.v.}}
\def\viz{{\em viz.}}
%
% andbreak  (for breaking author lists)
%
\def\andbreak{%% \begin{tabular}
\end{tabular}\\\begin{tabular}[t]{c}%% \end{tabular}
}
%
% titlequote
%
\def\titlequote#1{\hfill
\parbox{4in}{\begin{flushright}{\small\it #1}\end{flushright}}}
%
% weekdaystring
%
% Dump the day of the week in string form.
% This macro is only valid from 1901 A.D. through 2099 A.D.
%
\def\weekdaystring#1#2#3{{% extra brace saves enclosing register state
%
% days through the end of the year
% days := current year * 365
\count10=#3%
\multiply\count10 by 365%
% leap years := year / 4
\count11=#3%
\divide\count11 by 4%
% days := days + leap years
\advance\count10 by \count11
%
% find out if the current year is a leap year
% last leap year := leap years * 4
\count12=\count11%
\multiply\count12 by 4
% years since last leap year := current year - last leap year
\count13=#3%
\advance\count13 by -\count12%
% years since last leap year equals zero when current year is a leap year
%
% subtract off those days in this month and the following months
% days = days - following days [ is leap ] [ current month ]
\ifcase#2%
\or\ifcase\count13\advance\count10 by -366% leap January
\else\advance\count10 by -365% normal January
\fi%
\or\ifcase\count13\advance\count10 by -335% leap February
\else\advance\count10 by -334% normal February
\fi%
\or\advance\count10 by -306% March
\or\advance\count10 by -275% April
\or\advance\count10 by -245% May
\or\advance\count10 by -214% June
\or\advance\count10 by -184% July
\or\advance\count10 by -153% August
\or\advance\count10 by -122% September
\or\advance\count10 by -92% October
\or\advance\count10 by -61% November
\or\advance\count10 by -31% December
\fi%
%
% update days by day of month
% days := days + current day
\advance\count10 by #1%
%
% find weekday number
% offset for initial day of the week
\advance\count10 by 5
% last monday := (current day / 7) * 7
\count14=\count10%
\divide\count14 by 7%
\multiply\count14 by 7
% weekday number := current day - last monday
\count15=\count10%
\advance\count15 by -\count14
%
% now dump out appropriate string
\ifcase\count15 Monday\or Tuesday\or Wednesday%
\or Thursday\or Friday\or Saturday\or Sunday\fi%
}}
%
% monthstring
%
% Dump the month in string form.
%
\def\monthstring#1{\ifcase#1\or January\or February\or March\or April\or May%
\or June\or July\or August\or September\or October\or November\or December\fi}
%
% dateWDMY
%
% Redefine \today as "weekdaystring daynumber monthstring yearnumber" format.
%
\def\dateWDMY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\number\day\space\monthstring{\month}\space\number\year}}
%
% dateDMY
%
% Redefine \today as "daynumber monthstring yearnumber" format.
%
\def\dateDMY{\def\today{\number\day\space\monthstring{\month}%
\space\number\year}}
%
% dateWMDY
%
% Redefine \today as "weekdaystring monthstring daynumber, yearnumber" format.
%
\def\dateWMDY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\monthstring{\month}\space\number\day,\space\number\year}}
%
% dateMDY
%
% Redefine \today as "monthstring daynumber, yearnumber" format.
%
\def\dateMDY{\def\today{\monthstring{\month}\space\number\day,%
\space\number\year}}
%
% dateMY
%
% Redefine \today as "monthstring yearnumber" format.
%
\def\dateMY{\def\today{\monthstring{\month}\space\number\year}}
%
% dateY
%
% Redefine \today as "yearnumber" format.
%
\def\dateY{\def\today{\number\year}}

